Adaptive Message Quantization and Parallelization for Distributed Full-graph GNN Training

Distributed full-graph training of Graph Neural Networks (GNNs) over large graphs is bandwidth-demanding and time-consuming. Frequent exchanges of node features, embeddings and embedding gradients (all referred to as messages) across devices bring significant communication overhead for nodes with remote neighbors on other devices (marginal nodes) and unnecessary waiting time for nodes without remote neighbors (central nodes) in the training graph. This paper proposes an efficient GNN training system, AdaQP, to expedite distributed full-graph GNN training. We stochastically quantize messages transferred across devices to lower-precision integers for communication traffic reduction and advocate communication-computation parallelization between marginal nodes and central nodes. We provide theoretical analysis to prove fast training convergence (at the rate of O(T^{-1}) with T being the total number of training epochs) and design an adaptive quantization bit-width assignment scheme for each message based on the analysis, targeting a good trade-off between training convergence and efficiency. Extensive experiments on mainstream graph datasets show that AdaQP substantially improves distributed full-graph training's throughput (up to 3.01 X) with negligible accuracy drop (at most 0.30%) or even accuracy improvement (up to 0.19%) in most cases, showing significant advantages over the state-of-the-art works.

==> sections/5_implementation.tex <==
\section{Implementation Details}\label{sec:imp}

We build our system on top of DGL~\cite{wang2019deep} and PyTorch~\cite{paszke2019pytorch}, which leverages DGL for graph-related data storage and operations, uses PyTorch distributed package for process group's initialization and communication. Before training begins, DGL's built-in METIS algorithm partitions the graph, each training process is wrapped to only one device (GPU) and broadcasts the remote node indices (built from DGL's partition book) to create sending and receiving nodes index sets for fetching remote messages. The cost model for each device pair is also fitted in the preprocessing stage by sampling different communication volumes and their corresponding transmission time in each device pair. The index sets are stored once built to avoid repeated construction. To support the parallelization between the central graph's computation and the marginal graph's communication in both forward pass and backward pass, we integrate our customized  \textit{distributed graph aggregation layer} into PyTorch's Autograd mechanics. We use CPU thread event to synchronize the CUDA kernel launching on the central and marginal graph and use GPU CUDA event to synchronize the CUDA kernel execution, ensuring the GPU resources isolation proposed in Sec.\ref{sec:para}. For supporting extreme low bit-width messages compression and reducing the extra overhead to the lowest, we follow~\cite{liu2021exact} to implement the quantization/de-quantization CUDA kernels which merge all the quantized messages with lower precision (4-bit, or even 2-bit) into uniform 8-bit byte streams (supported data type of PyTorch). To transfer multiple bit-width quantized messages and match them with corresponding buffers, we first group messages according to their assigned bit-width, perform single bit-width quantization to each group and then concatenate all groups into a byte array before the transfer begins. After communication, each training process recovers full-precision messages from the byte array base on a bit-retrieval index set maintained and updated by the Adaptive Bit-width Assigner.

